Cyber-Risks in Paper Voting

Paper ballot voting with its fully-reviewable paper-trail is usually considered as more secure than their e-voting counterparts, given the large number of recent incidents. In this work, we explore the security of paper voting and show that paper voting, as it is implemented today, is surprisingly vulnerable to cyber-attacks. In particular, the aggregation methods of preliminary voting results of various countries rely on insecure communication channels like telephone, fax or non-secure e-mail. Furthermore, regulations typically do not mandate the use of secure channels for the transmission of preliminary results. We illustrate that preliminary results, despite their temporary nature, may have a severe impact on real-world decisions during the 3 to 30 days window until the final results are declared. An attacker exploiting this discrepancy can, e.g., benefit from stock market manipulation or call into question the legitimacy of the elections. This work investigates the cyber-risks in paper voting in a systematic manner by reviewing procedures in several countries (Estonia, France, Germany, the United Kingdom, and the United States of America) and through a comprehensive case-study of Switzerland. We examine the transmission systems currently in use through inquires from election officials. Moreover, we illustrate the feasibility of attacks by analyzing the frequent historical discrepancies between preliminary and final results. Considering our results and recent reports about easily modifiable preliminary results in Germany and the Netherlands, we conjecture similar weaknesses in other countries as well.

==> research/questions/eac.tex <==
- What do you do? From your website, we know certification and support including guidelines for election officials. 
- Are you involved in the process of  transmitting voting results from the counties/precincts to the state government? Do you know how states usually (or specific) do that? Are there "secure" systems in place?
- Are there anywhere official preliminary results transmission system in place? How many states are doing this? How about private companies doing this?
- I see on TV usually the results days before the official result is fixed. How does that work? Exit polls? 



==> research/questions/email.tex <==
Dear Elections Office

We are conducting an international survey on the transmission of voting results. We are interested in the general process of transmitting the result of ballot votes from the casting entity (e.g., voting office) to the federal level. We would like to ask you to answer the following questions:

- How does accumulation of single votes/ballots occurs, once they are cast? For example, do you have single voting computers and the results are somewhere central collected, or do you conduct ballot votes where the ballots are counted by multiple parties (e.g., counties) individually? Or is there another mechanism in place? Specifically, how are the voting results collected and added up? How do these results reach the next instance?

- What are the time limits in which the officials results are publicly announced? How Long does it usually take from the day the ballot voting ends?

- Does the state publish preliminary results based on incomplete information from its counties?
- If yes, what is the time within the first preliminary result is published, counting from the day the ballot voting ends?

- Do private companies collect preliminary results for the preliminary projection of the voting outcome? Are they published, e.g., in newspaper? How do these private companies collect this data?

- If yes, How many days are usually passed between the closing of the ballot boxes and the publication of the preliminary results collected by private companies?


Kind regards
Moritz Schneider
Institut für Informationssicherheit
ETH Zürich

CNB F 103.1
Universitätstrasse 6
8092 Zürich
Switzerland


==============
United Kingdom
==============

Dear Electoral Commission

We are conducting an international survey on the transmission of voting results. We are interested in the general process of transmitting the result of ballot votes from the casting entity (e.g., voting office) to the national level. We already looked at the law in the United Kingdom, more specifically at "Representation of the People Act 1983" and its updates in the recent years. However, we would like to ask you a few questions on some additional details:

- We read that, after the vote, the ballots are physically transported to the next central counting office and then they are counted at that location. Are there multiple central counting offices per constituency or is there only one? If there are multiple, how are the partial results transmitted and accumulated? Additionally, the votes must be accumulated across the country for a referendum. How does this work? How are the partial results transmitted?

- What are the time limits in which the officials results are publicly announced? How Long does it usually take from the day the ballot voting ends?

- Does the constituency publish preliminary results based on incomplete information from its central counting offices?
- If yes, how quickly are the first preliminary result usually published, counting from the day the ballot voting ends?

- Do private companies collect preliminary results for the preliminary projection of the voting outcome? Are they published, e.g., in newspaper? How do these private companies collect this data?

- If yes, How many days are usually passed between the closing of the ballot boxes and the publication of the preliminary results collected by private companies?


Kind regards
David Sommer
Institut für Informationssicherheit
ETH Zürich

CNB F 107.1
Universitätstrasse 6
8092 Zürich
Switzerland

===========
France
===========

Dear Elections Office

We are conducting an international survey on the transmission of voting results. We are interested in the general process of transmitting the result of ballot votes from the casting entity (e.g., voting office) to the federal level. We would like to ask you to answer the following questions:

- How does accumulation of single votes/ballots occurs, once they are cast? For example, are the ballots counted somewhere central, or are they counted in each individual county? Or is there another mechanism in place? Specifically, how are the voting results collected and added up? How do these results reach the next instance?

- What are the time limits in which the officials results are publicly announced? How Long does it usually take from the day the ballot voting ends?

- Does the state publish preliminary results based on incomplete information from its counties?
- If yes, what is the time within the first preliminary result is published, counting from the day the ballot voting ends?

- According to our knowledge, in France, it is forbidden to publish any statistics on the election on election day. However, there are belguim and swiss news outlets that do publish preliminary results. Do you know how these interim results are collected? Does the state communicate preliminary results to newspapers or do private companies collect preliminary results? If they are collected by private companies, how do these private companies collect this data?

Kind regards
David Sommer
Institut für Informationssicherheit
ETH Zürich

CNB F 107.1
Universitätstrasse 6
8092 Zürich
Switzerland



==============
France translated
==============
Monsieur, Madame du bureau d’élection

Je suis un chercheur de l'École polytechnique fédérale de Zurich en Suisse. Nous menons une étude internationale sur la transmission des résultats électoraux. Nous nous intéressons en particulier au processus général de transmission des résultats de vote par bulletin du bureau de vote au niveau national. Je vous serais très reconnaissant si vous pouviez répondre aux questions suivantes:

- Comment se produit l'accumulation des votes/bulletins uniques, une fois qu'ils ont été exprimés? Par exemple, les bulletins de vote sont-ils comptés à un endroit central ou dans chaque comté? Ou y a-t-il un autre mécanisme en place? Plus précisément, comment les résultats du vote sont-ils recueillis et additionnés? Comment ces résultats parviennent-ils à l'instance supérieure?

- Quels sont les délais dans lesquels les résultats officiels sont annoncés publiquement? Combien de temps s'écoule-t-il habituellement depuis le jour où le vote  prend fin? 

- L'État publie-t-il des résultats préliminaires basés sur des informations incomplètes provenant de ses comtés?
- Dans l'affirmative, quel est le délai de publication du premier résultat préliminaire, à compter du jour où le scrutin prend fin?

- A notre connaissance, en France, il est interdit de publier des statistiques sur les élections le jour du scrutin. Cependant, il existe des médias belges et suisses qui publient des résultats préliminaires. Savez-vous comment ces résultats intermédiaires sont recueillis? L'Etat communique-t-il des résultats préliminaires aux journaux ou les entreprises privées recueillent-elles des résultats préliminaires? S'ils sont recueillis par des entreprises privées, comment ces entreprises privées recueillent-elles ces données?

Je vous remercie sincèrement de votre temps et votre effort.

Avec mes meilleures salutations
Moritz Schneider
Institut pour la sécurité de l’information 
École polytechnique fédérale de Zurich

CNB F 103.1
Universitätstrasse 6
8092 Zürich
Switzerland

==============
Estonia
==============

Dear Elections Office

We are conducting an international survey on the transmission of voting results. We are interested in the general process of transmitting the result of ballot votes from the casting entity (e.g., voting office) to the national level. We already looked at the law in Estonia, more specifically at "Riigikogu Election Act". However, we would like to ask you a few questions on some additional details:

- We read that, after the vote, the ballot boxes are opened and the votes are counted. Is this happening at every voting office? Or are the ballots boxes transported to a counting office? 

- In §57.13 of the "Riigikogu Election Act" it is specified that the voting results are publicly announced by the voting district committee. How exactly is this announcement made? 

- For a referendum the entire country can vote for or against a certain case (e.g. "2003 Estonian European Union membership referendum"). How are the partial results from the counties transmitted to a central counting office that then accumulates the votes and declares the outcome? In many other countries there are two ways of communication: An official report with signatures from the voting committee, transmitted by post or electronic measures, and a fast electronic report for preliminary results. The preliminary results are used by newspapers or TV stations to provide projections and interim results. Is there a similar procedure in Estonia? Could you provide some details on the electronic transmission if there is such thing?

- What are the time limits in which the officials results are publicly announced? How Long does it usually take from the day the ballot voting ends until the outcome is final? If there are preliminary results, how fast are the first preliminary result usually published?

- Do private companies collect preliminary results for the preliminary projection of the voting outcome? Are they published, e.g., in newspapers? How do these private companies collect this data?

- If yes, How many days are usually passed between the closing of the ballot boxes and the publication of the preliminary results collected by private companies?

Kind regards
David Sommer
Institut für Informationssicherheit
ETH Zürich

CNB F 107.1
Universitätstrasse 6
8092 Zürich
Switzerland

==> research/questions/germany.tex <==
\begin{itemize}
    \item Schnellmeldungen werde fuer die voruebergehenden Resultate am Wahltag benuetzt. Die Wahlniederschrift mit den Unterschriften wird einige Tage spaeter das definitive Wahlergebniss liefern. Stimmt das so?
    \item Wie werden die Schnellmeldungen uebermittelt? Email? Telefon? Wer bestimmt das? Gibt es übersichten über alle Bundesländer?
    \item Authentifikation bei den Schnellmeldungen?
    \item Wird die Software PC-Wahl immer noch gebraucht?
    \item Wann werden die amtlichen Wahlergebnisse normalerweise publiziert? Welche Granularität? Wer publiziert was?
    \item Gab es jemals eine grundlegend andere Entscheidung nach der Schnellmeldung verglichen mit den amtlichen Wahlergebnissen?
    \item 
\end{itemize}


Email an Bundeswahlleiter:


